Electroweak Precision Observables in the Minimal Supersymmetric Standard Model

The current status of electroweak precision observables in the Minimal Supersymmetric Standard Model (MSSM) is reviewed. We focus in particular on the $W$ boson mass, M_W, the effective leptonic weak mixing angle, sin^2 theta_eff, the anomalous magnetic moment of the muon, (g-2)_\mu, and the lightest CP-even MSSM Higgs boson mass, m_h. We summarize the current experimental situation and the status of the theoretical evaluations. An estimate of the current theoretical uncertainties from unknown higher-order corrections and from the experimental errors of the input parameters is given. We discuss future prospects for both the experimental accuracies and the precision of the theoretical predictions. Confronting the precision data with the theory predictions within the unconstrained MSSM and within specific SUSY-breaking scenarios, we analyse how well the data are described by the theory. The mSUGRA scenario with cosmological constraints yields a very good fit to the data, showing a clear preference for a relatively light mass scale of the SUSY particles. The constraints on the parameter space from the precision data is discussed, and it is shown that the prospective accuracy at the next generation of colliders will enhance the sensitivity of the precision tests very significantly.

==> paperdef.tex <==
\catcode`@=11
\def\citer{\@ifnextchar [{\@tempswatrue\@citexr}{\@tempswafalse\@citexr[]}}
 
\def\@citexr[#1]#2{\if@filesw\immediate\write\@auxout{\string\citation{#2}}\fi
  \def\@citea{}\@cite{\@for\@citeb:=#2\do
    {\@citea\def\@citea{--\penalty\@m}\@ifundefined
       {b@\@citeb}{{\bf ?}\@warning
       {Citation `\@citeb' on page \thepage \space undefined}}%
\hbox{\csname b@\@citeb\endcsname}}}{#1}}
\catcode`@=12

%\renewcommand{\topfraction}{1.0}
%\renewcommand{\bottomfraction}{0.3}
\renewcommand{\textfraction}{0}
\renewcommand{\floatpagefraction}{1.0}

% new commands for cross referencing
%\def\refeq#1{\mbox{(\ref{#1})}}
\def\refeq#1{\mbox{eq.~(\ref{#1})}}
\def\refeqs#1{\mbox{eqs.~(\ref{#1})}}
\def\reffi#1{\mbox{Fig.~\ref{#1}}}
\def\reffis#1{\mbox{Figs.~\ref{#1}}}
\def\refta#1{\mbox{Tab.~\ref{#1}}}
%\def\refta#1{\mbox{Table~\ref{#1}}}
\def\reftas#1{\mbox{Tabs.~\ref{#1}}}
%\def\reftas#1{\mbox{Tables~\ref{#1}}}
\def\refse#1{\mbox{Sect.~\ref{#1}}}
\def\refses#1{\mbox{Sects.~\ref{#1}}}
%\def\refse#1{\mbox{Section~\ref{#1}}}
\def\refapp#1{\mbox{App.~\ref{#1}}}
%\def\refapp#1{\mbox{Appendix~\ref{#1}}}
\def\citere#1{\mbox{Ref.~\cite{#1}}}
\def\citeres#1{\mbox{Refs.~\cite{#1}}}

\newcommand{\mst}{m_{\tilde{t}}}
\newcommand{\delmst}{\Delta\mst}
\newcommand{\mstr}{m_{\tilde{t}_R}}
\newcommand{\mstl}{m_{\tilde{t}_L}}
\newcommand{\mste}{m_{\tilde{t}_1}}
\newcommand{\mstz}{m_{\tilde{t}_2}}
\newcommand{\msti}{m_{\tilde{t}_i}}
\newcommand{\mstip}{m_{\tilde{t}_{i'}}}
\newcommand{\mstj}{m_{\tilde{t}_j}}
\newcommand{\msb}{m_{\tilde{b}}}
\newcommand{\msbr}{m_{\tilde{b}_R}}
\newcommand{\msbl}{m_{\tilde{b}_L}}
\newcommand{\msbe}{m_{\tilde{b}_1}}
\newcommand{\msbz}{m_{\tilde{b}_2}}
\newcommand{\msbi}{m_{\tilde{b}_i}}
\newcommand{\msbj}{m_{\tilde{b}_j}}
\newcommand{\MstL}{M_{\tilde{t}_L}}
\newcommand{\MstR}{M_{\tilde{t}_R}}
\newcommand{\MsbL}{M_{\tilde{b}_L}}
\newcommand{\MsbR}{M_{\tilde{b}_R}}
\newcommand{\MsqL}{M_{\tilde{q}_L}}
\newcommand{\MsqR}{M_{\tilde{q}_R}}
\newcommand{\Mtlr}{M_{t}^{LR}}
\newcommand{\Mtlrz}{\KL M_{t}^{LR}\KR^2}
\newcommand{\Mtlrd}{\KL M_{t}^{LR}\KR^3}
\newcommand{\Mtlrv}{\KL M_{t}^{LR}\KR^4}
\newcommand{\Mtlrf}{\KL M_{t}^{LR}\KR^5}
\newcommand{\Mtlrse}{\KL M_{t}^{LR}\KR^6}
\newcommand{\Mtlrsi}{\KL M_{t}^{LR}\KR^7}
\newcommand{\Mtlra}{\KL M_{t}^{LR}\KR^8}
\newcommand{\Mblr}{M_{b}^{LR}}
\newcommand{\Mblrz}{\KL M_{b}^{LR}\KR^2}
\newcommand{\Mqlr}{M_{q}^{LR}}
\newcommand{\At}{A_t}
\newcommand{\Ab}{A_b}
\newcommand{\Atau}{A_\tau}
\newcommand{\Aq}{A_q}
\newcommand{\Ac}{A_c}
\newcommand{\As}{A_s}
\newcommand{\Xt}{X_t}
\newcommand{\Xb}{X_b}
\newcommand{\Xq}{X_q}
\newcommand{\Xc}{X_c}
\newcommand{\Xs}{X_s}

\newcommand{\mf}{m_f}
\newcommand{\mfp}{m_{f'}}
\newcommand{\mfi}{m_{f_i}}
\newcommand{\msfr}{m_{\tilde{f}_R}}
\newcommand{\msfl}{m_{\tilde{f}_L}}
\newcommand{\msf}{m_{\tilde{f}}}
\newcommand{\msfi}{m_{\tilde{f}_i}}
\newcommand{\msfe}{m_{\tilde{f}_1}}
\newcommand{\msfz}{m_{\tilde{f}_2}}
\newcommand{\Msl}{M_{\tilde{l}}}

\newcommand{\ms}{M_S}
\newcommand{\msusy}{M_{\rm SUSY}}
\newcommand{\msq}{m_{\tilde{q}}}
\newcommand{\msqi}{m_{\tilde{q}_i}}
\newcommand{\msqip}{m_{\tilde{q}_{i'}}}
\newcommand{\msqj}{m_{\tilde{q}_j}}
\newcommand{\msqe}{m_{\tilde{q}_1}}
\newcommand{\msqz}{m_{\tilde{q}_2}}

\newcommand{\sfn}{\tilde{f}}
\newcommand{\sfl}{\tilde{f}_L}
\newcommand{\sfr}{\tilde{f}_R}
\newcommand{\sfe}{\tilde{f}_1}
\newcommand{\sfz}{\tilde{f}_2}
\newcommand{\sfi}{\tilde{f}_i}
\newcommand{\sfj}{\tilde{f}_j}
\newcommand{\sfez}{\tilde{f}_{12}}
\newcommand{\sfze}{\tilde{f}_{21}}
\newcommand{\neone}{\tilde{\chi}^0_1}
\newcommand{\netwo}{\tilde{\chi}^0_2}
\newcommand{\chone}{\tilde{\chi}^+_1}
\newcommand{\chonem}{\tilde{\chi}^-_1}
\newcommand{\chtwo}{\tilde{\chi}^+_2}
\newcommand{\chtwom}{\tilde{\chi}^-_2}


\newcommand{\Hi}{H_i}
\newcommand{\cHe}{\cH_1}
\newcommand{\cHz}{\cH_2}
\newcommand{\Pe}{\phi_1}
\newcommand{\Pz}{\phi_2}
\newcommand{\Pez}{\phi_{1,2}}
\newcommand{\PePz}{\phi_1\phi_2}
\newcommand{\mpe}{m_{\Pe}}
\newcommand{\mpz}{m_{\Pz}}
\newcommand{\mpez}{m_{\PePz}}

\newcommand{\smallz}{{\scriptscriptstyle Z}} %  a smaller Z
\newcommand{\smallD}{{\scriptscriptstyle D}} %
\newcommand{\smallQ}{{\scriptscriptstyle Q}} %
\newcommand{\smallU}{{\scriptscriptstyle U}} %

\newcommand{\SU}{\mathrm {SUSY}}
\newcommand{\SM}{\mathrm {SM}}
\newcommand{\hi}{\mathrm {Higgs}}
\def\Liz#1{{\rm Li}_2 \KL #1 \KR}
\newcommand{\msbar}{$\overline{\rm{MS}}$}
\newcommand{\msbarm}{\overline{\rm{MS}}}
\newcommand{\drbar}{$\overline{\rm{DR}}$}
\newcommand{\drbarm}{\overline{\rm{DR}}}
\newcommand{\oa}{{\cal O}(\alpha)}
\newcommand{\oas}{{\cal O}(\alpha_s)}
\newcommand{\oaas}{{\cal O}(\alpha\alpha_s)}
\newcommand{\ogmzmts}{{\cal O}(\gf^2\mt^6)}
\def\order#1{${\cal O}(#1)$}
\def\orderm#1{{\cal O}\KL #1 \KR}
\newcommand{\cp}{{\cal CP}}
\newcommand{\cA}{{\cal A}}
\newcommand{\cH}{{\cal H}}
\newcommand{\cHi}{{\cal H}_i}
\newcommand{\cL}{{\cal L}}
\newcommand{\cO}{{\cal O}}
\newcommand{\cZ}{{\cal Z}}
\newcommand{\wz}{\sqrt{2}}
\newcommand{\edz}{\frac{1}{2}}
\def\ed#1{\frac{1}{#1}}
\newcommand{\twol}{two-loop}
\newcommand{\onel}{one-loop}
\newcommand{\mma}{{\em Mathematica}}
\newcommand{\tc}{{\em TwoCalc}}
\newcommand{\fa}{{\em FeynArts}}
\newcommand{\fh}{{\em FeynHiggs}}
\newcommand{\fhf}{{\em FeynHiggsFast}}
\newcommand{\shp}{{\em subhpole}}
\newcommand{\rp}{$\rho\,$-parameter}

\newcommand{\MW}{M_W}
\newcommand{\MZ}{M_Z}
\newcommand{\MA}{M_A}
\newcommand{\mh}{m_h}
\newcommand{\mH}{m_H}
\newcommand{\Mh}{M_h}
\newcommand{\MH}{M_H}
\newcommand{\mhmax}{m_h^{\rm max}}
\newcommand{\mHp}{m_{H^\pm}}
\newcommand{\MHp}{M_{H^\pm}}
\newcommand{\mG}{m_G}
\newcommand{\mGp}{m_{G^\pm}}
\newcommand{\MHSM}{M_H^{\SM}}
\newcommand{\mhtree}{m_{h,{\rm tree}}}
\newcommand{\mHtree}{m_{H,{\rm tree}}}
\newcommand{\tadH}{T_H}
\newcommand{\tadh}{T_h}
\newcommand{\tadA}{T_A}
\newcommand{\tadG}{T_G}
\newcommand{\tanb}{\tan \beta\,}
\newcommand{\sinb}{\sin \beta\,}
\newcommand{\cosb}{\cos \beta\,}
\newcommand{\sinbsq}{\sin^2 \!\beta\,}
\newcommand{\cosbsq}{\cos^2 \!\beta\,}
\newcommand{\sina}{\sin \alpha\,}
\newcommand{\cosa}{\cos \alpha\,}
\newcommand{\tana}{\tan \alpha\,}
\newcommand{\sinasq}{\sin^2 \!\alpha\,}
\newcommand{\cosasq}{\cos^2 \!\alpha\,}

\newcommand{\sudxsuzxue}{SU(3)_C \otimes SU(2)_L \otimes U(1)_Y}
\newcommand{\suzxue}{SU(2)_L \otimes U(1)_Y}

\newcommand{\dr}{\De\rho}
\newcommand{\mt}{m_{t}}
\newcommand{\mtexp}{m_{t}^{\rm exp}}
\newcommand{\Mt}{M_{t}}
\newcommand{\mtms}{\overline{m}_t}
\newcommand{\mq}{m_{q}}
\newcommand{\mb}{m_{b}}
\newcommand{\Mb}{M_{b}}
\newcommand{\mc}{m_{c}}
\newcommand{\gl}{\tilde{g}}
\newcommand{\Mgl}{m_{\tilde{g}}}
\newcommand{\mgl}{m_{\tilde{g}}}
\newcommand{\Sferm}{\tilde{f}}
\newcommand{\Sfermp}{\tilde{f}'}
\newcommand{\sq}{\tilde{q}}
\newcommand{\sqi}{\tilde{q}_i}
\newcommand{\sqj}{\tilde{q}_j}
\newcommand{\sql}{\tilde{q}_L}
\newcommand{\sqr}{\tilde{q}_R}
\newcommand{\sqe}{\tilde{q}_1}
\newcommand{\sqz}{\tilde{q}_2}
\newcommand{\sqez}{\tilde{q}_{12}}
\newcommand{\Stop}{\tilde{t}}
\newcommand{\StopL}{\tilde{t}_L}
\newcommand{\StopR}{\tilde{t}_R}
\newcommand{\Stope}{\tilde{t}_1}
\newcommand{\Stopz}{\tilde{t}_2}
\newcommand{\Stopi}{\tilde{t}_i}
\newcommand{\Stopj}{\tilde{t}_j}
\newcommand{\Sbot}{\tilde{b}}
\newcommand{\SbotL}{\tilde{b}_L}
\newcommand{\SbotR}{\tilde{b}_R}
\newcommand{\Sbote}{\tilde{b}_1}
\newcommand{\Sbotz}{\tilde{b}_2}
\newcommand{\Sboti}{\tilde{b}_i}
\newcommand{\Sbotj}{\tilde{b}_j}
\newcommand{\Stau}{\tilde{\tau}}
\newcommand{\Snet}{\tilde{\nu}_\tau}
\newcommand{\Smu}{\tilde \mu}
\newcommand{\Sneum}{\tilde \nu_\mu}
\newcommand{\Scha}{\tilde{c}}
\newcommand{\SchaL}{\tilde{c}_L}
\newcommand{\SchaR}{\tilde{c}_R}
\newcommand{\Sstr}{\tilde{s}}
\newcommand{\SstrL}{\tilde{s}_L}
\newcommand{\SstrR}{\tilde{s}_R}
\newcommand{\tiu}{\tilde u}
\newcommand{\tid}{\tilde d}
\newcommand{\tiq}{\tilde q}
\newcommand{\dst}{\Delta_{\tilde{t}}}
\newcommand{\tst}{\theta_{\tilde{t}}}
\newcommand{\tsb}{\theta_{\tilde{b}}}
\newcommand{\tsf}{\theta\kern-.20em_{\tilde{f}}}
\newcommand{\tsfp}{\theta\kern-.20em_{\tilde{f}\prime}}
\newcommand{\tsq}{\theta\kern-.15em_{\tilde{q}}}
\newcommand{\sw}{s_W}
\newcommand{\swq}{s_W^2}
\newcommand{\cw}{c_W}
\newcommand{\cwq}{c_W^2}
\newcommand{\sweff}{\sin^2\theta_{\mathrm{eff}}}
\newcommand{\aef}{a_{\rm eff}^f}
\newcommand{\vef}{v_{\rm eff}^f}

\newcommand{\cha}[1]{\tilde \chi^\pm_{#1}}
\newcommand{\neu}[1]{\tilde \chi^0_{#1}}

\newcommand{\sintt}{\sin\tst}
\newcommand{\sinQtt}{\sin^2\tst}
\newcommand{\sinZtt}{\sin 2\tst}
\newcommand{\sinQZtt}{\sin^2 2\tst}
\newcommand{\sintb}{\sin\tsb}
\newcommand{\sinQtb}{\sin^2\tsb}
\newcommand{\sinZtb}{\sin 2\tsb}
\newcommand{\sintf}{\sin\tsf}
\newcommand{\sintfp}{\sin\tsfp}
\newcommand{\sinQtf}{\sin^2\tsf}
\newcommand{\sinZtf}{\sin 2\tsf}
\newcommand{\sintq}{\sin\tsq}
\newcommand{\sinQtq}{\sin^2\tsq}
\newcommand{\sinZtq}{\sin 2\tsq}

\newcommand{\costt}{\cos\tst}
\newcommand{\cosQtt}{\cos^2\tst}
\newcommand{\cosZtt}{\cos 2\tst}
\newcommand{\costb}{\cos\tsb}
\newcommand{\cosQtb}{\cos^2\tsb}
\newcommand{\cosZtb}{\cos 2\tsb}
\newcommand{\costf}{\cos\tsf}
\newcommand{\costfp}{\cos\tsfp}
\newcommand{\cosQtf}{\cos^2\tsf}
\newcommand{\cosZtf}{\cos 2\tsf}
\newcommand{\costq}{\cos\tsq}
\newcommand{\cosQtq}{\cos^2\tsq}
\newcommand{\cosZtq}{\cos 2\tsq}

\newcommand{\stt}{s_{\tilde{t}}}
\newcommand{\stb}{s_{\tilde{b}}}
\newcommand{\stf}{s_{\tilde{f}}}
\newcommand{\stq}{s_{\tilde{q}}}
\newcommand{\ctt}{c_{\tilde{t}}}
\newcommand{\ctb}{c_{\tilde{b}}}
\newcommand{\ctf}{c_{\tilde{f}}}
\newcommand{\ctq}{c_{\tilde{q}}}

\newcommand{\KL}{\left(}
\newcommand{\KR}{\right)}
\newcommand{\KKL}{\left[}
\newcommand{\KKR}{\right]}
\newcommand{\KKKL}{\left\{}
\newcommand{\KKKR}{\right\}}
\newcommand{\BL}{\lbrack}
\newcommand{\BR}{\rbrack}

\newcommand{\VL}{\left( \begin{array}{c}}
\newcommand{\VR}{\end{array} \right)}
\newcommand{\ML}{\left( \begin{array}{cc}}
\newcommand{\MLd}{\left( \begin{array}{ccc}}
\newcommand{\MLv}{\left( \begin{array}{cccc}}
\newcommand{\MR}{\end{array} \right)}
\newcommand{\dd}{\partial}
\newcommand{\dmu}{\partial_{\mu}}
\newcommand{\dmo}{\partial^{\mu}}
\newcommand{\mn}{{\mu\nu}}
\newcommand{\hc}{\mbox {h.c.}}
\newcommand{\re}{\mbox {Re}\,}
\newcommand{\OP}{\omega_+}
\newcommand{\OM}{\omega_-}
\newcommand{\Tb}{\tan \beta\hspace{1mm}}
\newcommand{\tb}{\tan \beta}
\newcommand{\TQb}{\tan^2 \beta\hspace{1mm}}
\newcommand{\CTb}{\cot \beta\hspace{1mm}}
\newcommand{\CTQb}{\cot^2 \beta\hspace{1mm}}
%\newcommand{\Sb}{\sin \beta\hspace{1mm}}
\newcommand{\sbe}{\sin \beta\hspace{1mm}}
\newcommand{\SQb}{\sin^2\beta\hspace{1mm}}
\newcommand{\SDb}{\sin^3\beta\hspace{1mm}}
\newcommand{\SVb}{\sin^4\beta\hspace{1mm}}
\newcommand{\Cb}{\cos \beta\hspace{1mm}}
\newcommand{\CQb}{\cos^2\beta\hspace{1mm}}
\newcommand{\CDb}{\cos^3\beta\hspace{1mm}}
\newcommand{\CVb}{\cos^4\beta\hspace{1mm}}
\newcommand{\Sa}{\sin \alpha\hspace{1mm}}
\newcommand{\SQa}{\sin^2\alpha\hspace{1mm}}
\newcommand{\Ca}{\cos \alpha\hspace{1mm}}
\newcommand{\CQa}{\cos^2\alpha\hspace{1mm}}
\newcommand{\Ta}{\tan\al}
\newcommand{\CTa}{\cot\al}
\newcommand{\Sab}{\sin (\alpha + \beta)\hspace{1mm}}
\newcommand{\Cab}{\cos (\alpha + \beta)\hspace{1mm}}
\newcommand{\Sba}{\sin (\beta - \alpha)\hspace{1mm}}
\newcommand{\Samb}{\sin (\al - \be)\hspace{1mm}}
\newcommand{\Cba}{\cos (\beta - \alpha)\hspace{1mm}}
\newcommand{\Camb}{\cos (\al - \be)\hspace{1mm}}
\newcommand{\SZa}{\sin 2\alpha\hspace{1mm}}
\newcommand{\SQZa}{\sin^2 2\alpha\hspace{1mm}}
\newcommand{\CZa}{\cos 2\alpha\hspace{1mm}}
\newcommand{\CQZa}{\cos^2 2\alpha\hspace{1mm}}
\newcommand{\SZb}{\sin 2\beta\hspace{1mm}}
\newcommand{\SQZb}{\sin^2 2\beta\hspace{1mm}}
\newcommand{\CZb}{\cos 2\beta\hspace{1mm}}
\newcommand{\CQZb}{\cos^2 2\beta\hspace{1mm}}
\newcommand{\CDZb}{\cos^3 2\beta\hspace{1mm}}
\newcommand{\CVZb}{\cos^4 2\beta\hspace{1mm}}
\newcommand{\CQba}{\cos^2 (\beta - \alpha)\hspace{1mm}}
\newcommand{\SQba}{\sin^2 (\beta - \alpha)\hspace{1mm}}
\newcommand{\SDba}{\sin^3 (\beta - \alpha)\hspace{1mm}}
\newcommand{\CQab}{\cos^2 (\alpha + \beta)\hspace{1mm}}
\newcommand{\SQab}{\sin^2 (\alpha + \beta)\hspace{1mm}}
\newcommand{\SDab}{\sin^3 (\alpha + \beta)\hspace{1mm}}
\newcommand{\SDea}{\sin \De\al}
\newcommand{\CDea}{\cos \De\al}
\newcommand{\CQDea}{\cos^2\De\al}
\newcommand{\TDea}{\tan \De\al}
\newcommand{\TQDea}{\tan^2\De\al}

\newcommand{\tev}{\,\, \mathrm{TeV}}
\newcommand{\gev}{\,\, \mathrm{GeV}}
\newcommand{\mev}{\,\, \mathrm{MeV}}

\newcommand{\BC}{\begin{center}}
\newcommand{\EC}{\end{center}}
\newcommand{\BE}{\begin{equation}}
\newcommand{\EE}{\end{equation}}
\newcommand{\BEA}{\begin{eqnarray}}
\newcommand{\BEAnn}{\begin{eqnarray*}}
\newcommand{\EEA}{\end{eqnarray}}
\newcommand{\EEAnn}{\end{eqnarray*}}
\newcommand{\non}{\nonumber}
\newcommand{\id}{{\rm 1\kern-.12em
\rule{0.3pt}{1.5ex}\raisebox{0.0ex}{\rule{0.1em}{0.3pt}}}}
\newcommand{\lsim}
{\;\raisebox{-.3em}{$\stackrel{\displaystyle <}{\sim}$}\;}
\newcommand{\gsim}
{\;\raisebox{-.3em}{$\stackrel{\displaystyle >}{\sim}$}\;}


\newcommand{\cf}{C_F}
\newcommand{\gf}{G_F}
\newcommand{\Gf}{G_F}
\newcommand{\GF}{G_F}
\newcommand{\nf}{N_f}
% shorthands for greek letters
\def\al{\alpha}
\def\aeff{\al_{\rm eff}}
\def\aeffapprox{\al_{\rm eff}{\rm (approx)}}
\newcommand{\Saeff}{\sin\aeff}
\newcommand{\Caeff}{\cos\aeff}
\newcommand{\sbaeff}{\sin(\be-\aeff)}
\newcommand{\sqbaeff}{\sin^2(\be-\aeff)}
\def\als{\alpha_s}
\def\alt{\alpha_t}
\def\alb{\alpha_b}
\def\altl{\alpha_{\rm 2-loop}}
\def\gs{g_s}
\def\be{\beta}
\def\ben{\be_0}
\def\bee{\be_1}
\def\bez{\be_2}
\def\ga{\gamma}
\def\gan{\ga_0}
\def\gae{\ga_1}
\def\gaz{\ga_2}
\def\de{\delta}
\def\deqed{\de\Ga_\ga}
\def\eps{\varepsilon}
\def\la{\lambda}
\def\si{\sigma}
\def\ie{i\epsilon}
\def\om{\omega}
\def\ohsq{\Omega_\chi h^2}
\def\Ga{\Gamma}
\def\Gh{\Ga_h}
\def\GH{\Ga_H}
\def\Gz{\Ga_0}
\def\Ge{\Ga_1}
\def\Geeff{\Ga_{1,\rm eff}}
\def\Geg{\Ga_{1,g}}
\def\Gga{\Ga_\ga}
\def\Gg{\Ga_g}
\def\Ggl{\Ga_{\gl}}
\def\Gtot{\Ga_{\rm tot}}
\def\De{\Delta}
\def\La{\Lambda}
\def\Laqcd{\La_{\rm QCD}}
\def\Si{\Sigma}
\def\Sip{\Sigma'}
\def\Sie{\Sigma^{(1)}}
\def\Siz{\Sigma^{(2)}}
\def\Sii{\Sigma^{(i)}}
\def\Siep{\Sigma'^{(1)}}
\def\Sizp{\Sigma'^{(2)}}
\def\Siip{\Sigma'^{(i)}}

\def\hSi{\hat{\Sigma}}
\newcommand{\se}[1]{\Sigma_{#1}}
\newcommand{\ser}[1]{\hat{\Sigma}_{#1}}
\def\hSip{\hat{\Sigma}'}
\def\hSie{\hat{\Sigma}^{(1)}}
\def\hSiz{\hat{\Sigma}^{(2)}}
\def\hSiep{\hat{\Sigma}^{(1)}'}
\def\hSizp{\hat{\Sigma}^{(2)}'}
\def\hSiH{\hSi_{HH}}
\def\hSih{\hSi_{hh}}
\def\hSihH{\hSi_{hH}}
\def\hSipH{\hSip_{HH}}
\def\hSiph{\hSip_{hh}}
\def\hSiphH{\hSip_{hH}}
\def\hSieh{\hSie_{h}}
\def\hSieH{\hSie_{H}}
\def\hSiehH{\hSie_{hH}}
\def\hSizh{\hSiz_{h}}
\def\hSizH{\hSiz_{H}}
\def\hSizhH{\hSiz_{hH}}
\newcommand{\htad}{\hat{t}}
\newcommand{\tade}{t^{(1)}}
\newcommand{\tadz}{t^{(2)}}

\newcommand{\dmZsq}{\delta M_Z^2}
\newcommand{\dMZsq}{\delta \MZ^2}
\newcommand{\dmWsq}{\delta m_W^2}
\newcommand{\dMWsq}{\delta \MW^2}
\newcommand{\dmhsq}{\delta m_h^2}
\newcommand{\dmhHsq}{\delta m_{hH}^2}
\newcommand{\dmHhsq}{\delta m_{Hh}^2}
\newcommand{\dmhGsq}{\delta m_{hG}^2}
\newcommand{\dmhAsq}{\delta m_{hA}^2}
\newcommand{\dmHsq}{\delta m_H^2}
\newcommand{\dmHGsq}{\delta m_{HG}^2}
\newcommand{\dmHAsq}{\delta m_{HA}^2}
\newcommand{\dmAsq}{\delta m_A^2}
\newcommand{\dmAGsq}{\delta m_{AG}^2}
\newcommand{\dmGsq}{\delta m_G^2}
\newcommand{\dmHpmsq}{\delta m_{H^\pm}^2}
\newcommand{\dmHmGpsq}{\delta m_{H^- G^+}^2}
\newcommand{\dmGmHpsq}{\delta m_{G^- H^+}^2}
\newcommand{\dmGpmsq}{\delta m_{G^\pm}^2}

\newcommand{\dtadH}{\delta T_H}
\newcommand{\dtadh}{\delta T_h}
\newcommand{\dtadA}{\delta T_A}

\newcommand{\dtanb}{\delta\!\tan\!\beta\,}
\newcommand{\dZ}[1]{\delta Z_{#1}}

\newcommand{\Ph}{\mathswitchr h}
\newcommand{\PH}{\mathswitchr H}

\newcommand{\deMZe}{\de \MZ^{2\,(1)}}
\newcommand{\deMZz}{\de \MZ^{2\,(2)}}
\newcommand{\deMZi}{\de \MZ^{2\,(i)}}
\newcommand{\deMAe}{\de \MA^{2\,(1)}}
\newcommand{\deMAz}{\de \MA^{2\,(2)}}
\newcommand{\deMAi}{\de \MA^{2\,(i)}}
\newcommand{\deZHie}{\de Z_{H_i}^{(1)}}
\newcommand{\deZHiz}{\de Z_{H_i}^{(2)}}
\newcommand{\deZHee}{\de Z_{H_1}^{(1)}}
\newcommand{\deZHez}{\de Z_{H_1}^{(2)}}
\newcommand{\deZHze}{\de Z_{H_2}^{(1)}}
\newcommand{\deZHzz}{\de Z_{H_2}^{(2)}}
\newcommand{\deTbe}{\de\Tb^{(1)}}
\newcommand{\deTbz}{\de\Tb^{(2)}}
\newcommand{\detie}{\de t_i^{(1)}}
\newcommand{\detiz}{\de t_i^{(2)}}
\newcommand{\detee}{\de t_1^{(1)}}
\newcommand{\detez}{\de t_1^{(2)}}
\newcommand{\detei}{\de t_1^{(i)}}
\newcommand{\detze}{\de t_2^{(1)}}
\newcommand{\detzz}{\de t_2^{(2)}}
\newcommand{\detzi}{\de t_2^{(i)}}
\newcommand{\deVie}{\de V_i^{(1)}}
\newcommand{\deViz}{\de V_i^{(2)}}
\newcommand{\deVee}{\de V_{\Pe}^{(1)}}
\newcommand{\deVez}{\de V_{\Pe}^{(2)}}
\newcommand{\deVei}{\de V_{\Pe}^{(i)}}
\newcommand{\deVze}{\de V_{\Pz}^{(1)}}
\newcommand{\deVzz}{\de V_{\Pz}^{(2)}}
\newcommand{\deVzi}{\de V_{\Pz}^{(i)}}
\newcommand{\deVeze}{\de V_{\PePz}^{(1)}}
\newcommand{\deVezz}{\de V_{\PePz}^{(2)}}
\newcommand{\deVezi}{\de V_{\PePz}^{(i)}}


\newcommand{\SLASH}[2]{\makebox[#2ex][l]{$#1$}/}
\newcommand{\Dslash}{\SLASH{D}{.5}\,}
\newcommand{\dslash}{\SLASH{\dd}{.15}}
\newcommand{\kslash}{\SLASH{k}{.15}}
\newcommand{\pslash}{\SLASH{p}{.2}}
\newcommand{\qslash}{\SLASH{q}{.08}}

\newcommand{\sqmsmt}{\sqrt{\ms^2-\mt^2}}
\newcommand{\sqmsmtbar}{\sqrt{\ms^2-\mtms^2}}
\newcommand{\lmtms}{\KL\frac{\mt^2}{\ms^2}\KR}
\newcommand{\lmtmsms}{\KL\frac{\mtms^2}{\ms^2}\KR}
\newcommand{\lmsmt}{\KL\frac{\ms^2 - \mt^2}{\mt^2}\KR}

\newcommand{\lc}{linear collider}
\newcommand{\epem}{$e^+e^-$}
\newcommand{\eetohZhA}{$e^+e^- \to hZ,hA$}
\newcommand{\eetohZ}{$e^+e^- \to hZ$}
\newcommand{\eetohA}{$e^+e^- \to hA$}
\newcommand{\ipb}{$\mbox{pb}^{-1}$}
\newcommand{\ifb}{$\mbox{fb}^{-1}$}
\newcommand{\iab}{$\mbox{ab}^{-1}$}
\newcommand{\gvf}{g_V^f}
\newcommand{\gaf}{g_A^f}
\newcommand{\AFB}{A_{\rm FB}}
\newcommand{\ALR}{A_{\rm LR}}

\newcommand{\plane}[2]{$#1$--$#2$~plane}
%\newcommand{\plane}[2]{($#1, #2$)~plane}

\newcommand{\br}{{\rm BR}}
\newcommand{\hff}{h \to f\bar{f}}
\newcommand{\Hff}{H \to f\bar{f}}
\newcommand{\hbb}{h \to b\bar{b}}
\newcommand{\Hbb}{H \to b\bar{b}}
\newcommand{\htautau}{h \to \tau^+\tau^-}
\newcommand{\hcc}{h \to c\bar{c}}
\newcommand{\rf}{R_f}
\newcommand{\hmumu}{h \to \mu^+\mu^-}
\newcommand{\mumuh}{\mu^+ \mu^- \to h}
\newcommand{\hWW}{h \to WW^*}
\newcommand{\WWh}{WW \to h}
\newcommand{\WWH}{WW \to H}
\newcommand{\hgg}{h \to gg}
\newcommand{\hgaga}{h \to \ga\ga}
\newcommand{\gagah}{\ga \ga \to h}
\newcommand{\staustauH}{\Staue\AStaue \to H}
%\newcommand{\cff}{C_{ff}}
\newcommand{\cff}{C_f^{(u)}}
%\newcommand{\cfpfp}{C_{f'f'}}
\newcommand{\cfpfp}{C_f^{(d)}}
\newcommand{\Zh}{Z_h}
\newcommand{\wZh}{\sqrt{\Zh}}
\newcommand{\ZH}{Z_H}
\newcommand{\wZH}{\sqrt{\ZH}}
\newcommand{\ZhH}{Z_{hH}}
\newcommand{\ZHh}{Z_{Hh}}
\newcommand{\Zext}{\cZ^{\rm ext}}
\newcommand{\Zmix}{\cZ^{\rm mix}}
\newcommand{\rS}{{\rm S\,}}
\newcommand{\rP}{{\rm P\,}}
\def\ul#1{\underline{\vphantom{g}#1}}

\newcommand{\amu}{a_\mu}
\newcommand{\amuX}{a_\mu^{\chi,{\rm 2L}}}
\newcommand{\amuSUoL}{a_\mu^{\rm SUSY,1L}}
\newcommand{\amuexp}{a_\mu^{\rm exp}}
\newcommand{\amutheo}{a_\mu^{\rm theo}}
\newcommand{\amuMSSM}{a_\mu^{\rm MSSM}}
\newcommand{\amuMSSMtl}{a_\mu^{\rm MSSM, 2L}}
\newcommand{\amuSUbos}{a_\mu^{\rm bos,2L, MSSM}}
\newcommand{\SUbos}{{\rm bos,2L, MSSM}}
\newcommand{\delamu}{\De\amu^{\rm 2L}}

\newcommand{\mpar}[1]{\marginpar{\tiny #1}}
\def\mua{\marginpar[\boldmath\hfil$\uparrow$]%
                   {\boldmath$\uparrow$\hfil}%
                    \typeout{marginpar: $\uparrow$}\ignorespaces}
\def\mda{\marginpar[\boldmath\hfil$\downarrow$]%
                   {\boldmath$\downarrow$\hfil}%
                    \typeout{marginpar: $\downarrow$}\ignorespaces}
\def\mla{\marginpar[\boldmath\hfil$\rightarrow$]%
                   {\boldmath$\leftarrow $\hfil}%
                    \typeout{marginpar: $\leftrightarrow$}\ignorespaces}
\def\Mua{\marginpar[\boldmath\hfil$\Uparrow$]%
                   {\boldmath$\Uparrow$\hfil}%
                    \typeout{marginpar: $\Uparrow$}\ignorespaces}
\def\Mda{\marginpar[\boldmath\hfil$\Downarrow$]%
                   {\boldmath$\Downarrow$\hfil}%
                    \typeout{marginpar: $\Downarrow$}\ignorespaces}
\def\Mla{\marginpar[\boldmath\hfil$\Rightarrow$]%
                   {\boldmath$\Leftarrow $\hfil}%
                    \typeout{marginpar: $\Leftrightarrow$}\ignorespaces}
\newcommand{\todo}[1]{\mbox{}\\ {\bf XXXXXXXXXXXXXXXXXXXXXXXXXXXXXXX}\\
                      {\bf #1}\\{\bf XXXXXXXXXXXXXXXXXXXXXXXXXXXXXXX}\\
                      \mbox{}\\}                 



%**********************************
%   new from Hollik



 \newcommand{\Li}{{\rm Li}}
 \newcommand{\elevenbf}{\bf}
 \newcommand{\elevenit}{\it}
 \newcommand{\beq}{\begin{equation}}
 \newcommand{\eeq}{\end{equation}}
 \newcommand{\bea}{\begin{eqnarray}}
 \newcommand{\eea}{\end{eqnarray}}
 \newcommand{\barr}{\begin{array}}
 \newcommand{\earr}{\end{array}}
 \newcommand{\bc}{\begin{center}}
 \newcommand{\ec}{\end{center}}
 \newcommand{\btab}{\begin{tabular}}
 \newcommand{\etab}{\end{tabular}}
 \newcommand{\gv}{\mbox{GeV}}
 \newcommand{\tv}{\mbox{TeV}}
 \newcommand{\mv}{\mbox{MeV}}
 \newcommand{\nn}{\nonumber}
 \newcommand{\ra}{\rightarrow}
 \newcommand{\lra}{\leftrightarrow}
 \newcommand{\ipi}{\frac{i}{16\pi^2}}
 \newcommand{\dkm}{\mu^{4-D} \int \frac{d^Dk}{(2\pi)^D} }
 \newcommand{\dkk}{[k^2-m^2]}
 \newcommand{\dkq}{[(k+q)^2-m^2]}
 %\newcommand{\Dkk}{[k^2-m^2]}
 %\newcommand{\Dkq}{[(k+q)^2-m^2]}
 \newcommand{\sg}{\Sigma^{\gamma\gamma}}
 \newcommand{\sz}{\Sigma^{Z}}
 %\newcommand{\swwoh}{\Sigma^{W}}
 \newcommand{\sgz}{\Sigma^{\gamma Z}}
 \newcommand{\szr}{\hat{\Sigma}^{Z}}
 \newcommand{\szzr}{\hat{\Sigma}^{ZZ}}
 \newcommand{\swwr}{\hat{\Sigma}^{WW}}
 \newcommand{\sgzr}{\hat{\Sigma}^{\gamma Z}}
 \newcommand{\sggr}{\hat{\Sigma}^{\gamma\gamma}}
 \newcommand{\dmz}{\frac{\delta M_Z^2}{M_Z^2}}
 \newcommand{\dmw}{\frac{\delta M_W^2}{M_W^2}}
 \newcommand{\dmmz}{\delta M_Z^2}
 \newcommand{\dmmw}{\delta M_W^2}
 \newcommand{\mwb}{M_W^{0\,2}}
 \newcommand{\mzb}{M_Z^{0\,2}}
 \newcommand{\mzoo}{M_{Z_0}^2}
 \newcommand{\mzop}{M_{Z'}^2}
 \newcommand{\dro}{\Delta\rho}
 \newcommand{\droz}{\Delta\rho_{Z'}}
 \newcommand{\drb}{\Delta\overline{\rho}}
 \newcommand{\drot}{\Delta\rho(top)}
 \newcommand{\drou}{(\Delta\rho)_{univ}}
 \newcommand{\dron}{(\Delta\rho)}
 \newcommand{\drob}{\Delta\rho_b^{(t)}}
% \newcommand{\al}{\alpha}
 \newcommand{\alpi}{\frac{\alpha}{4\pi}}
 \newcommand{\api}{\frac{\alpha}{\pi}}
 \newcommand{\aspi}{\frac{\alpha_{\rm s}}{\pi}}
 \newcommand{\alfs}{\frac{\alpha^2}{4s}}
 \newcommand{\alspi}{\frac{\alpha_s}{\pi}}
 \newcommand{\ap}{\frac{\alpha}{2\pi}}
 \newcommand{\m}{\mu}
 \newcommand{\g}{\gamma}
% \newcommand{\G}{\Gamma}
 \newcommand{\Gmu}{G_{\mu}}
 \newcommand{\gamu}{\gamma_{\mu}}
 \newcommand{\gimu}{\gamma^{\mu}}
 \newcommand{\ganu}{\gamma_{\nu}}
 \newcommand{\ginu}{\gamma^{\nu}}
 \newcommand{\giro}{\gamma^{\rho}}
 \newcommand{\gisi}{\gamma^{\sigma}}
 \newcommand{\garo}{\gamma_{\rho}}
 \newcommand{\gasi}{\gamma_{\sigma}}
 \newcommand{\gafi}{\gamma_5}
% \newcommand{\La}{\Lambda}
 \newcommand{\Lr}{\hat{\Lambda}}
 \newcommand{\Gu}{\Gamma_{\mu}}
 \newcommand{\Gr}{\hat{\Gamma}_{\mu}}
 \newcommand{\Pig}{\Pi^{\gamma}}
 \newcommand{\Pigr}{\hat{\Pi}^{\gamma}}
 \newcommand{\Pizr}{\hat{\Pi}^Z}
 \newcommand{\Pir}{\hat{\Pi}}
 \newcommand{\Pgrz}{\hat{\Pi}^{\gamma}(M_Z^2)}
 \newcommand{\Pgzrz}{\hat{\Pi}^{\gamma Z}(M_Z^2)}
 \newcommand{\Pzrz}{\hat{\Pi}^Z(M_Z^2)}
 \newcommand{\sgr}{\hat{\Sigma}^{\gamma}}
 \newcommand{\noi}{\noindent}
 \newcommand{\epmf}{e^+e^- \rightarrow f\bar{f}}
 \newcommand{\epmm}{e^+e^- \rightarrow \mu^+\mu^-}
 \newcommand{\epmb}{e^+e^- \rightarrow b\bar{b}}
 \newcommand{\epm}{e^+e^-}
 \newcommand{\vae}{v_e a_e}
 \newcommand{\vaf}{v_f a_f}
 \newcommand{\vvf}{v_e v_f}
 \newcommand{\aaf}{a_e a_f}
 \newcommand{\ve}{(v_e^2+a_e^2)}
 \newcommand{\vf}{(v_f^2+a_f^2)}
 \newcommand{\vff}{(v_f^2+a_f^2-4\mu_f a_f^2)}
 \newcommand{\vam}{(v_e^2-a_e^2)}
 \newcommand{\gve}{(g_{\rm V}^{e\,2}+g_{\rm A}^{e\,2})}
% \newcommand{\gvf}{(g_{\rm V}^{f\,2}+g_{\rm A}^{f\,2})}
 \newcommand{\rchi}{\mbox{Re}\,\chi_Z^0(s)}
 \newcommand{\chiz}{\mid\chi_Z^0(s) \mid^2}
 \newcommand{\rc}{radiative corrections }
% \newcommand{\sm}{Standard Model }
 \newcommand{\sm}{SM}
 \newcommand{\su}{SU(2)$\times$U(1) }
 \newcommand{\siw}{\sin^2\theta_W}
 \newcommand{\cow}{\cos^2\theta_W}
 \newcommand{\sinw}{\sin\theta_W}
 \newcommand{\cosw}{\cos\theta_W}
 \newcommand{\sinm}{\sin\theta_{\rm M}}
 \newcommand{\sinmm}{\sin^2\theta_{\rm M}}
 \newcommand{\cosm}{\cos\theta_{\rm M}}
 \newcommand{\cosmm}{\cos^2\theta_{\rm M}}
 \newcommand{\swo}{s_W^{0\,2}}
 \newcommand{\cwo}{c_W^{0\,2}}
 \newcommand{\swb}{\overline{s}_W^{\,2}}
 \newcommand{\cwb}{\overline{c}_W^2}
 \newcommand{\seff}{\sin^2\theta_f}
 %\newcommand{\sefl}{\sin^2\theta_{eff}^{\,l}}
 \newcommand{\sefl}{\sin^2\theta_e}
 \newcommand{\snue}{(1-4\sin^2\!\theta_{\!\nu e})}
 \newcommand{\dal}{\Delta\alpha}
 \newcommand{\dalms}{\Delta\hat{\alpha}}
 \newcommand{\pgz}{\frac{\Pi_{\gamma Z}(s)}
                        {1+\Pi_{\gamma\gamma}(s)} }
 \newcommand{\irg}{s+\hat{\Sigma}^{\gamma\gamma}(s)}
 \newcommand{\irz}{s-m_Z^2+\hat{\Sigma}^{ZZ}(s)}
 \newcommand{\irrg}{\frac{1}{s+\hat{\Sigma}^{\gamma\gamma}}}
 \newcommand{\irrz}{\frac{1}{s-m_Z^2+\hat{\Sigma}^{ZZ}}}
 \newcommand{\mixx}{\left( \hat{\Sigma}^{\gamma Z} \right) ^2}
 \newcommand{\mixs}{\left( \hat{\Sigma}^{\gamma Z}(s) \right) ^2}
 \newcommand{\sirr}{\hat{\Sigma}^{ZZ}_{(2)}}
 \newcommand{\imsirr}{\mbox{Im }\hat{\Sigma}^Z_{(2)}}
 \newcommand{\mz}{M_Z^2}
 \newcommand{\mw}{M_W^2}
 \newcommand{\mwphys}{m_{W,phys}^2}
 \newcommand{\smw}{m_W^2}
 \newcommand{\smz}{m_Z^2}
 \newcommand{\mm}{\hat{m}_Z^2}
 \newcommand{\gm}{\hat{\Gamma}_Z^2}
 \newcommand{\bul}{\bullet}
 \newcommand{\real}{\mbox{Re}}
 \newcommand{\Imag}{\mbox{Im}}
 \newcommand{\Dr}{\Delta r}
 \newcommand{\Drb}{\overline{\Delta r}}
 \newcommand{\iprop}{s-m_Z^2+i\frac{s}{m_Z}\Gamma_Z}
 \newcommand{\prop}{\frac{1}{s-m_Z^2+i\frac{s}{m_Z}\Gamma_Z}}
 \newcommand{\fge}{F^{\gamma e}}
 \newcommand{\fze}{F^{Z e}}
 \newcommand{\fgf}{F^{\gamma f}}
 \newcommand{\fzf}{F^{Z f}}
 \newcommand{\isw}{\frac{1}{(2s_W)^2}}
 \newcommand{\gir}{\gamma_{IR}}
 \newcommand{\gfin}{\gamma_{fin}}
 \newcommand{\vgg}{V^{\gamma\gamma}}
 \newcommand{\vgz}{V^{\gamma Z}}
 \newcommand{\agg}{A^{\gamma\gamma}}
 \newcommand{\agz}{A^{\gamma Z}}
% \newcommand{\bee}{\beta_e}
 \newcommand{\bef}{\beta_f}
 \newcommand{\bint}{\beta_{int}}
 \newcommand{\mzs}{m^2-s}
% \newcommand{\eps}{\epsilon}
 \newcommand{\veps}{\varepsilon}
 %\newcommand{\api}{\frac{2\alpha}{\pi}}
 \newcommand{\alp}{\frac{\alpha}{2\pi}}
 \newcommand{\qef}{Q_eQ_f}
 \newcommand{\dlog}{\mbox{Li}_2}
 \newcommand{\oal}{O(\alpha^2)}
 \newcommand{\alr}{A_{\rm LR}}
 \newcommand{\afb}{A_{\rm FB}}
 \newcommand{\apol}{A_{\rm FB}^{\rm pol}}
 \newcommand{\apolf}{A_{\rm FB}^{\rm pol}(e^+e^- \rightarrow f\bar{f})}
 \newcommand{\apolm}{A_{\rm FB}^{\rm pol}(e^+e^- \rightarrow \mu^+\mu^-)}
 \newcommand{\afbm}{A_{\rm FB}(e^+e^- \rightarrow \mu^+\mu^-)}
 \newcommand{\as}{asymmetry }
 \newcommand{\ass}{asymmetries }
 \newcommand{\dz}{\delta Z}
 \newcommand{\dzl}{\delta Z_L^{(\ell)}}
 \newcommand{\ren}{renormalization constant }
 \newcommand{\rens}{renormalization constants }
 \newcommand{\ksl}{\not k}
 \newcommand{\summ}{m_1^2+m_2^2}
 \newcommand{\difm}{m_1^2-m_2^2}
 \newcommand{\up}{\frac{8}{3}}
 \newcommand{\dow}{\frac{4}{3}}
% \newcommand{\gl}{\frac{1-\gamma_5}{2}}
 \newcommand{\gr}{\frac{1+\gamma_5}{2}}
 \newcommand{\plus}{\phi^+}
 \newcommand{\mis}{\phi^-}
 \newcommand{\nul}{\phi^0}
 \newcommand{\adnu}{\overline{\nu}}
 \newcommand{\adl}{\overline{l}}
 \newcommand{\lept}{\frac{m_l}{m_W}\cdot\tan\beta}
 \newcommand{\lepto}{\frac{m_l}{m_W}}
 \newcommand{\adu}{\overline{u}}
 \newcommand{\add}{\overline{d}}
 \newcommand{\lyu}{{\cal L}_{\rm Yukawa}}
 \newcommand{\bsw}{\overline{s_W^2}}
 \newcommand{\oag}{O\left(\frac{\alpha}{\pi}\,
                   \frac{\Gamma_Z}{m_Z}\right)}
 \newcommand{\mzo}{m_{Z0}^2}
 \newcommand{\mwo}{m_{W0}^2}
 \newcommand{\jme}{J^{(e)}}
 \newcommand{\jmf}{J^{(f)}}
 \newcommand{\jmef}{J^{(e)\, 5}}
 \newcommand{\jmff}{J^{(f)\, 5}}
 \newcommand{\jmm}{J^{(\mu)}}
 \newcommand{\jmeb}{\bar{J}^{(e)}}
 \newcommand{\jmfb}{\bar{J}^{(f)}}
 \newcommand{\jcce}{J_{CC}^{(e)}}
 \newcommand{\jccf}{J_{CC}^{(f)}}
 \newcommand{\est}{e_*^2}
 \newcommand{\sst}{s_*^2}
 \newcommand{\Gst}{G_{\mu *}}
 \newcommand{\rst}{\rho_*}
 \newcommand{\Gzst}{\Gamma_{*Z}}
 \newcommand{\Gwst}{\Gamma_{*W}}
 \newcommand{\ecst}{\frac{e^2_*}{s^2_* c_*^2}}
 \newcommand{\esst}{\frac{e^2_*}{s_*^2}}
 \newcommand{\mwst}{\frac{e^2_*}{s^2_*}\,\frac{1}
                   {4\sqrt{2} G_{\mu *}}}
 \newcommand{\mzst}{\frac{e^2_*}{s^2_* c^2_*}\,\frac{1}
                   {4\sqrt{2} G_{\mu *}\rho_*}}
 \newcommand{\Dh}{\hat{D}}
 \newcommand{\pr}{{\it Phys.\ Rev.\ }}
 \newcommand{\zp}{{\it Z.\ Phys.\ }}
 \newcommand{\pl}{{\it Phys.\ Lett.\ }}
 \newcommand{\prl}{{\it Phys.\ Rev.\ Lett.\ }}
 \newcommand{\np}{{\it Nucl.\ Phys.\ }}
 \newcommand{\plb}{{\it Phys.\ Lett.\ }}
 \newcommand{\prd}{{\it Phys.\ Rev.\  }}
 %\newcommand{\pr}{Phys.\ Rev.\ }
 %\newcommand{\prd}{Phys.\ Rev.\ D }
 %\newcommand{\zp}{Z.\ Phys.\ C }
 %\newcommand{\pl}{Phys.\ Lett.\ }
 %\newcommand{\prl}{Phys.\ Rev.\ Lett.\ }
 %\newcommand{\np}{Nucl.\ Phys.\ B }
 \newcommand{\ctanw}{\frac{c_W^2}{s_W^2}}
 \newcommand{\gfa}{\frac{\sqrt{2}G_{\mu}m_W^2}{16\pi^2}}
 \newcommand{\deltaw}{\Deltavar-\log\frac{m_W^2}{\mu^2}}
 \newcommand{\deltz}{\Deltavar-\log\frac{m_Z^2}{\mu^2}}
 \newcommand{\deltaz}{\Deltavar-\log\frac{m_Z^2}{\mu^2}
                      +\frac{5}{3} }
 \newcommand{\deltat}{\Deltavar-\log\frac{m_t^2}{\mu^2} }
 \newcommand{\deltak}{\Deltavar-\log\frac{k^2}{\mu^2} }
 \newcommand{\fvge}{F_{\rm V}^{\g e}}
 \newcommand{\fage}{F_{\rm A}^{\g e}}
 \newcommand{\fvze}{F_{\rm V}^{Z  e}}
 \newcommand{\faze}{F_{\rm A}^{Z  e}}
 \newcommand{\fvgf}{F_{\rm V}^{\g f}}
 \newcommand{\fagf}{F_{\rm A}^{\g f}}
 \newcommand{\fvzf}{F_{\rm V}^{Z  f}}
 \newcommand{\fazf}{F_{\rm A}^{Z  f}}
 \newcommand{\dkap}{\Delta\kappa}
 \newcommand{\vev}{vacuum expectation value }
 \newcommand{\sth}{s_{\theta}}
 \newcommand{\cth}{c_{\theta}}
 \newcommand{\sell}{s_{\ell}^2}
% \newcommand{\stt}{s_{\theta}^2}
 \newcommand{\Rnu}{R_{\nu}}
 \newcommand{\Rnub}{R_{\bar{\nu}}}
 \newcommand{\sne}{s^2_{\nu e}}
 \newcommand{\cne}{c^2_{\nu e}}
 \newcommand{\sms}{\hat{s}^2}
 \newcommand{\cms}{\hat{c}^2}
 \newcommand{\smsb}{\hat{s}}
 \newcommand{\cmsb}{\hat{c}}
 \newcommand{\roms}{\hat{\rho}}
 \newcommand{\Drms}{\Delta\hat{r}}
 \newcommand{\ems}{\hat{e}}
% \newcommand{\ms}{\overline{MS}}
 \newcommand{\xms}{X_{\overline{MS}}}
 \newcommand{\dvb}{\hat{\delta}_{VB}}
 %\newcommand{\ams}{\alfa_{\overline{MS}}}
 \newcommand{\ams}{\hat{\alpha}}
 \newcommand{\mvms}{\hat{m}_V^2}
 \newcommand{\mwms}{\hat{m}_W^2}
 \newcommand{\mzms}{\hat{m}_Z^2}
 \newcommand{\dk}{\frac{d^4k}{(2\pi)^4}}
 %\newcommand{\dkm}{\mu^{4-D} \int \frac{d^Dk}{(2\pi)^D} }
 %\newcommand{\dkk}{[k^2-m^2]}
 %\newcommand{\dkq}{[(k+q)^2-m^2]}
 \newcommand{\Dkk}{[k^2-m_1^2]}
 \newcommand{\Dkq}{[(k+q)^2-m_2^2]}
 \newcommand{\Dkp}{[(k+p_1)^2-m_2^2]}
 \newcommand{\Dkr}{[(k+p_1+p_2)^2-m_3^2]}
 \newcommand{\km}{k_{\mu}}
 \newcommand{\kmn}{k_{\mu}k_{\nu}}
 \newcommand{\ppm}{p_1^{\mu}}
 \newcommand{\pqm}{p_2^{\mu}}
 \newcommand{\ppn}{p_1^{\nu}}
 \newcommand{\pqn}{p_2^{\nu}}
 \newcommand{\pps}{p_1^2}
 \newcommand{\pqs}{p_2^2}
 \newcommand{\prs}{p_3^2}
 \newcommand{\ppq}{(p_1p_2)}
 \newcommand{\imag}{{\cal I}m}


\makeatletter

\newcount\@tempcntc
\def\@citex[#1]#2{\if@filesw\immediate\write\@auxout{\string\citation{#2}}\fi
  \@tempcnta\z@\@tempcntb\m@ne\def\@citea{}\@cite{\@for\@citeb:=#2\do
    {\@ifundefined
       {b@\@citeb}{\@citeo\@tempcntb\m@ne\@citea
        \def\@citea{,\penalty\@m\ }{\bf ?}\@warning
       {Citation `\@citeb' on page \thepage \space undefined}}%
    {\setbox\z@\hbox{\global\@tempcntc0\csname
b@\@citeb\endcsname\relax}%
     \ifnum\@tempcntc=\z@ \@citeo\@tempcntb\m@ne
       \@citea\def\@citea{,\penalty\@m}
       \hbox{\csname b@\@citeb\endcsname}%
     \else
      \advance\@tempcntb\@ne
      \ifnum\@tempcntb=\@tempcntc
      \else\advance\@tempcntb\m@ne\@citeo
      \@tempcnta\@tempcntc\@tempcntb\@tempcntc\fi\fi}}\@citeo}{#1}}

\def\@citeo{\ifnum\@tempcnta>\@tempcntb\else\@citea
  \def\@citea{,\penalty\@m}%
  \ifnum\@tempcnta=\@tempcntb\the\@tempcnta\else
   {\advance\@tempcnta\@ne\ifnum\@tempcnta=\@tempcntb \else
\def\@citea{--}\fi
    \advance\@tempcnta\m@ne\the\@tempcnta\@citea\the\@tempcntb}\fi\fi}

\makeatother



